Real-Time Open-Domain Question Answering with Dense-Sparse Phrase Index

Existing open-domain question answering (QA) models are not suitable for real-time usage because they need to process several long documents on-demand for every input query. In this paper, we introduce the query-agnostic indexable representation of document phrases that can drastically speed up open-domain QA and also allows us to reach long-tail targets. In particular, our dense-sparse phrase encoding effectively captures syntactic, semantic, and lexical information of the phrases and eliminates the pipeline filtering of context documents. Leveraging optimization strategies, our model can be trained in a single 4-GPU server and serve entire Wikipedia (up to 60 billion phrases) under 2TB with CPUs only. Our experiments on SQuAD-Open show that our model is more accurate than DrQA (Chen et al., 2017) with 6000x reduced computational cost, which translates into at least 58x faster end-to-end inference benchmark on CPUs.

==> 06-exp-f2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/fig3.pdf}
    \caption{F1 vs the ratio between document embedding \& phrase embedding when computing the final score, fixing the number of documents to 5. }
    \label{fig:ratio}
\end{figure}

==> 06-exp-f3.tex <==

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/fig4cl.pdf}
    \caption{This figure will be F1 vs latency (ms) (by varying number of documents) for three models: DrQA, base and large in the open-domain, with fixed tf-idf coefficient.}
    \label{fig:latency}
\end{figure}

==> 06-exp-t2.tex <==
\begin{table}[]
    \centering
    \resizebox{0.7\columnwidth}{!}{%
    \begin{tabular}{lcc}
        \toprule
                           & F1    & EM   \\
        \midrule
        \ours       & 79.1  & 70.5  \\
        $+$Linear after last layer       & X  & X  \\
        $+$Independent encoders       & X  & X  \\
        $-$Coherency scalar       & 71.5  & 81.5  \\
        \midrule
        \ours       & 38.0  & 30.0  \\
        $-$Dense       & X  & X  \\
        $-$Sparse       & X  & X  \\
        \bottomrule
        
    \end{tabular}
    }
    \caption{Model ablations in two settings: SQuAD v1.1 (top) and SQuAD-Open (bottom).}
    \label{tab:ab}
\end{table}

==> 90-nobert.tex <==

Here we describe a few ways to improve our basic encoder when we cannot benefit from pretrained model.

\paragraph{Sparse Representation} 

The goal of our sparse model is to obtain a sparse representation for start and end, $\sbo_{i:j} = [\sbo^1_i,\sbo^2_j] \in \mathbb{R}^{2D}$, where $D$ is very large (e.g. $D=100,000$) and each start and end sparse vector is sparsely activated.
Then the final phrase representation is obtained by concatenating both dense and sparse vectors, i.e. $[\pb_{i:j}, \sbo_{i:j}] \in \mathbb{R}^{2a + 2D}$. We obtain the start sparse vectors, $\Sb^1 = [\sbo^1_1;\dots;\sbo^1_T] \in \mathbb{R}^{T \times D}$, by

\begin{equation}
    \Sb^1 = \max(0, Q^1(\Db^1) K^1(\Db^1)^\top) \Xb
\end{equation}

where $Q^1, K^1 :\mathbb{R}^{T \times d} \rightarrow \mathbb{R}^{T \times d}$ are trainable functions, $\Db^1 \in \mathbb{R}^{T \times d}$ is the matrix of the dense start vectors from the text encoder, and $\Xb \in \mathbb{R}^{T \times D}$ is a one-hot vector of the input words over a vocabulary of size $D$.
Note that the ReLU activation ($\max(0, *)$) encourages sparse activation of the sparse vectors.
We obtain the sparse matrix for the end position, $\Sb^2$ in a similar manner, where we have independent trainable functions $Q^2, K^2$ over $\Db^2$.

Note that applying $Q,K$ on the dense vectors and dot producting them is analogous to obtaining logits for self-attention. However, instead of using softmax to normalize the attention, we use ReLU to sparsely activate the attention, and then sparsely map the attention to vocabulary space. Hence it can be viewed as a learned bag-of-word weight for each phrase.

There exist several possible choices for $Q, K$. Following \citet{piqa}, we use LSTM. Another option is a mutli-layer perceptron as in Transformer~\ms{cite}.

In order to perform inner product, we need a corresponding sparse vector the question.

If we do not handle the sparse vectors carefully (e.g. if we treat them as dense vectors), we will face memory inefficiency.

\paragraph{Multi-sense representation} We can benefit from having multiple ($M$) vectors per phrase. This is different from ensemble method because we are jointly training several phrase models for single question model. We obtain a loss for each phrase model and jointly minimize the average of the losses. At inference time, we store all vectors. While this increases the storage by $M$-fold, we can benefit better accuracy.

\paragraph{Dual task learning} We regularize training by trying to generate the original question from the target answer phrase's representation using seq2seq~\cite{}. 


==> _05-exp-f2.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/fig2.pdf}
    \caption{F1 vs average number of words that the model can cover per MB of storage. We control the storage with two methods: thresholding and phrase size. We clearly observe that both contribute to the trade-off between accuracy and storage, and further, when they are combined (green), we observe a better trade-off. The combined data point corresponds to PI-BERT* (127D) model.}
    \label{fig:f1byte}
\end{figure}

==> _05-exp-t3.tex <==

\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lcccc}
        \toprule
                            & \#P(M)         & \#W/s      & \multicolumn{2}{c}{ms/Q} \\
                            &    & GPU  & GPU & CPU   \\
        \midrule
        Baseline            & 10.6  & X  & X  & X \\
        Baseline+ELMo       & 16.8  & X  & X  & X \\
        \midrule
        \ours\ Base        & 118   & 2.88k  & 17  & 60 \\ 
        \ours\ Large       & 338   & 1.26k   & 33 & 222 \\
        \bottomrule
        
    \end{tabular}
    }
    \caption{\# of Model parameters in millions (\#P(M)), \# of words that a single P40 GPU can process to obtain phrase embeddings per second (\#W/s), and \# of milliseconds per query for embedding the question on a single thread of CPU.
             \#W/s and ms/Q are measured on PI-SQuAD and averaged. Note that the size and the speed of PI-BERT is almost independent of the phrase size, so we omit phrase-size-wise comparison.
             Batch sizes for base and large models are 16 and 4, respectively on P40.}
    \label{tab:pi-squad-stat}
\end{table}
